Adversarial Generation of Continuous Images

In most existing learning systems, images are typically viewed as 2D pixel arrays. However, in another paradigm gaining popularity, a 2D image is represented as an implicit neural representation (INR) - an MLP that predicts an RGB pixel value given its (x,y) coordinate. In this paper, we propose two novel architectural techniques for building INR-based image decoders: factorized multiplicative modulation and multi-scale INRs, and use them to build a state-of-the-art continuous image GAN. Previous attempts to adapt INRs for image generation were limited to MNIST-like datasets and do not scale to complex real-world data. Our proposed INR-GAN architecture improves the performance of continuous image generators by several times, greatly reducing the gap between continuous image GANs and pixel-based ones. Apart from that, we explore several exciting properties of the INR-based decoders, like out-of-the-box superresolution, meaningful image-space interpolation, accelerated inference of low-resolution images, an ability to extrapolate outside of image boundaries, and strong geometric prior. The project page is located at https://universome.github.io/inr-gan.

==> appendices/lowres-inference.tex <==
\section{Accelerated inference of low-resolution images}\label{ap:lowres-inference}

Several classifiers can produce a prediction faster when an input is easy to classify \cite{BranchyNet, MSDNet}.
A generative model should have a similar property: when we ask a model to generate an image of lower resolution than the model was trained on --- it should be able to do it faster.
However, traditional convolutional decoders lack this property: to produce a lower-resolution image, one would need to perform the full inference and then downsample the resulted image with standard interpolation techniques.
In contrast, INR-based decoders are capable of doing this naturally: for this, we should just evaluate them on a sparser grid compared to what they were trained on.
To state the claim rigorously, we compute an amount of multiply-accumulate (MAC) operations for our INR-based generator and StyleGAN2 generator trained on FFHQ $1024^2$ for different lower-resolution image sizes.
To produce the low-resolution image with StyleGAN2, we first produce the full-resolution image and them downsample it with nearest neighbour interpolation.
For our model, we just evaluate it on a grid of the given resolution.
The results are reported on ~\figref{fig:fast-lowres-generation}.
To the best of our knowledge, our work is the first one that explores the accelerated generation of lower-resolution images --- an analog of early-exit strategies \cite{BranchyNet} for classifier models for image generation task.

\input{figures/fast-lowres-generation}


==> appendices/training-on-top-of-weights.tex <==
\section{Training $\D$ on top of INR weights}\label{ap:training-D-on-top-of-weights}
In theory, one can train $\D$ on top of $\F$ weights since conversion of an ImageNet-sized dataset of images into a dataset of INRs can be done in several days, depending on the $\F$ architecture.
But such an approach has 3 severe downsides: 1) changing INR architecture would require re-converting the whole dataset severely restricting preliminary experimentation; 2) input size for $D$ inreases a lot 3) one inevitably loses information during the conversion process (INR reconstruction may not be perfect).
That's why we opt for training $D$ on top of real images.
We do this by evaluating $F_{\bm\theta}(\bm p)$ on each iteration at each pixel coordinate of $H \times W$ grid.
Our efficient INR implementation via batch matrix multiplication allows to make this process $\times 2$ times faster compared to an inference process of a traditional convolutional GAN of comparable size.


==> figures/imagenet-aspect-ratios.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/imagenet-aspect-ratios.pdf}
    \caption{ImageNet aspect ratios distribution. Despite the fact that real-world aspect ratios is very far from being ``squares'' --- modern works still train either on squares on fixed-size rectangles. That's why we propose to move towards free-shaped image generation and propose ImageNet-FS dataset: a dataset where images are not cropped to some fixed size but are left at their original aspect ratio. See appendix \ref{ap:imagenet-fs} for details.}
    \label{fig:imagenet-aspect-ratios}
\end{figure}


==> figures/inr-diagram.tex <==
\begin{figure}
\centering
\includegraphics[width=0.6\linewidth]{images/architectures/inr.pdf}
\caption{Illustration of an image represented in the implicit neural representation (INR) form $\F$, i.e. as an MLP that predicts an RGB pixel value given its $(x,y)$ coordinates.
In contrast to the pixel-based representation, it stores the image in its true continuous form. 
In our paper, we explore adversarial generation of images in such a representation.}
\label{fig:inr-diagram}
\end{figure}


==> figures/upsampled-fid.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/superresolution/upsampled-fid.pdf}
    \caption{\textbf{Upsampled FID} scores for different upsampling techniques. We train the model on LSUN Bedroom 128$\times$128 and then generate $2\times$ upsampled images with the corresponding upsampling technique. After that FID score is computed for LSUN bedroom $256 \times 256$ dataset.}
    \label{fig:upsampled-fid}
\end{figure}


==> tables/conv-vs-inr-decoders.tex <==
\begin{table}
\caption{Comparison between convolution-based and INR-based 2D image decoders. We define these properties in Section~\ref{sec:intro} and provide empirical evidence in Section~\ref{sec:experiments:properties}.}
\label{table:conv-vs-inr-decoders}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|cc|}
\hline
Property & Convolutions & INRs \\
\hline
Out-of-the-box superresolution & \ding{55} & \ding{51}  \\
Accelerated low-resolution inference & \ding{55} & \ding{51} \\
Geometric prior & \ding{55} & \ding{51} \\
Using local context information & \ding{51} & \ding{55}  \\
Extrapolating outside of image boundaries & \ding{55} & \ding{51} \\
% Using local context information & Yes & No  \\
\hline
\end{tabular}
}
\end{table}

